Assessing Network Operator Actions to Enhance Digital Sovereignty and Strengthen Network Resilience: A Longitudinal Analysis during the Russia-Ukraine Conflict

We conduct longitudinal and temporal analyses on active DNS measurement data to investigate how the Russia-Ukraine conflict impacted the network infrastructures supporting domain names under ICANN's CZDS new gTLDs. Our findings revealed changes in the physical locations of network infrastructures, utilization of managed DNS services, infrastructure redundancy, and distribution, which started right after the first reported Russian military movements in February 2022. We also found that domains from different countries had varying location preferences when moving their hosting infrastructure. These observed changes suggest that network operators took proactive measures in anticipation of an armed conflict to promote resilience and protect the sovereignty of their networks in response to the conflict.

==> graphics/tab_dns_loc.tex <==
\begin{table}[!h]
    \centering
    \setlength\tabcolsep{3pt}
    \def\arraystretch{1.3}
    \begin{tabular}{llrr}
    \toprule
    \textbf{Initial} & \textbf{Final} & \textbf{\# Unique domain} &   \textbf{\# Unique AS} \\
    \midrule
    \multirow{4}{*}{Full inside} & Full inside* &         112,734 &  1,291 (1.1\%) \\
              & Partial inside &           2,069 &   231 (11.2\%) \\
              & None inside** &          30,762 &    513 (1.7\%) \\
              & Not exist &         441,781 &       \\
    \cline{1-4}
    \multirow{4}{*}{Partial inside} & Full inside &          16,209 &    380 (2.3\%) \\
              & Partial inside &          16,035 &    500 (3.1\%) \\
              & None inside &          18,211 &    406 (2.2\%) \\
              & Not exist &         106,761 &       \\
    \cline{1-4}
    \multirow{4}{*}{None inside} & Full inside*** &          20,858 &    379 (1.8\%) \\
              & Partial inside &           4,258 &    283 (6.6\%) \\
              & None inside &       6,915,828 &  7,616 (0.1\%) \\
              & Not exist &      12,774,921 &       \\
    \cline{1-4}
    \multirow{3}{*}{Not exist} & Full inside &         466,289 &    937 (0.2\%) \\
              & Partial inside &          46,429 &    455 (1.0\%) \\
              & None inside &      15,674,524 &  5,828 (0.0\%) \\
    \bottomrule
    \multicolumn{4}{l}{\textit{*stayed inside the conflict area}} \\
    \multicolumn{4}{l}{\textit{**moved away from the conflict area}} \\ 
    \multicolumn{4}{l}{\textit{***moved in to the conflict area}} \\
    \hline
    \\
    \end{tabular}
    \caption{DNS location movement for in-depth analysis.}
    \label{tab:dns_loc_move}
\end{table}

==> graphics/tab_move_by_registrant.tex <==
\begin{tabular}{ccrrrrrrrrrr}
\toprule
   Initial & \begin{tabular}{c} Registrant\\ Country \end{tabular} &     RU &    US &   DE &    UA &   AU &   NL &   BR &  PL &  IE &  SK \\
% Initial & \begin{tabular}{c} Registrant\\ Country \end{tabular} &        &       &      &       &      &      &      &     &     &     \\
\midrule
\multirow{7}{*}{RU} & RU &  25,249 &  93\% &   3\% &   1\% &   0\% &   0\% &  2\% \\
   & US &   9,742 &  34\% &  32\% &  16\% &   0\% &  13\% &  2\% \\
   & IS &   1,925 &  14\% &  65\% &   9\% &   1\% &   0\% &  4\% \\
   & JP &   1,511 &   0\% &  24\% &  75\% &   0\% &   0\% &  0\% \\
   & UA &   1,204 &  37\% &  11\% &  11\% &  29\% &   0\% &  5\% \\
   & CN &   1,081 &   7\% &  47\% &  41\% &   0\% &   2\% &  0\% \\
   & PL &     719 &   0\% &   2\% &  82\% &   0\% &   0\% &  0\% \\
\cline{1-9}
\multirow{7}{*}{UA} & UA &   4,273 &   1\% &   3\% &   4\% &  86\% &   0\% &  2\% \\
   & US &   1,244 &   5\% &  43\% &  16\% &  15\% &  12\% &  5\% \\
   & IS &     496 &   1\% &  58\% &   7\% &  22\% &   1\% &  6\% \\
   & RU &     471 &  66\% &  10\% &   5\% &   9\% &   0\% &  5\% \\
   & JP &     240 &   0\% &  18\% &  81\% &   0\% &   0\% &  0\% \\
   & CN &     191 &   0\% &  56\% &  34\% &   1\% &   4\% &  0\% \\
   & PL &      84 &   0\% &   6\% &  65\% &   6\% &   0\% &  1\% \\
\bottomrule
\end{tabular}

==> graphics/tab_whois_host_country.tex <==
\begin{table}[]
    \centering
    
    \begin{tabular}{llrrrrrrrrrr}
    {} & {} & {RU} & {US} & {DE} & {UA} & {AU} & {NL} & {BR} & {PL} & {IE} & {SK} \\
    {Registrant Country} & {Initial} & {} & {} & {} & {} & {} & {} & {} & {} & {} & {} \\
    \multirow[c]{2}{*}{RU} & RU & \background-color#08306b \color#f1f1f1 13759 & \background-color#cadef0 \color#000000 413 & \background-color#cde0f1 \color#000000 195 & \background-color#f6faff \color#000000 10 & \background-color#f7fbff \color#000000 2 & \background-color#08306b \color#f1f1f1 232 & \background-color#08306b \color#f1f1f1 146 & \background-color#dfecf7 \color#000000 7 & \background-color#dae8f6 \color#000000 7 & \background-color#f7fbff \color#000000 0 \\
     & UA & \background-color#f5f9fe \color#000000 187 & \background-color#f4f9fe \color#000000 33 & \background-color#f5f9fe \color#000000 12 & \background-color#f5fafe \color#000000 25 & \background-color#f7fbff \color#000000 0 & \background-color#eef5fc \color#000000 10 & \background-color#ebf3fb \color#000000 9 & \background-color#f4f9fe \color#000000 1 & \background-color#f7fbff \color#000000 0 & \background-color#f7fbff \color#000000 0 \\
    \multirow[c]{2}{*}{CN} & RU & \background-color#f7fbff \color#000000 44 & \background-color#d5e5f4 \color#000000 313 & \background-color#bfd8ed \color#000000 251 & \background-color#f7fbff \color#000000 0 & \background-color#f5f9fe \color#000000 10 & \background-color#f5fafe \color#000000 2 & \background-color#e1edf8 \color#000000 16 & \background-color#f7fbff \color#000000 0 & \background-color#f7fbff \color#000000 0 & \background-color#f7fbff \color#000000 0 \\
     & UA & \background-color#f7fbff \color#000000 0 & \background-color#f1f7fd \color#000000 58 & \background-color#eff6fc \color#000000 37 & \background-color#f7fbff \color#000000 0 & \background-color#f6faff \color#000000 5 & \background-color#f7fbff \color#000000 0 & \background-color#f3f8fe \color#000000 3 & \background-color#f7fbff \color#000000 0 & \background-color#f7fbff \color#000000 0 & \background-color#f7fbff \color#000000 0 \\
    \multirow[c]{2}{*}{UA} & RU & \background-color#f4f9fe \color#000000 265 & \background-color#eef5fc \color#000000 83 & \background-color#e5eff9 \color#000000 83 & \background-color#e4eff9 \color#000000 210 & \background-color#f7fbff \color#000000 0 & \background-color#dce9f6 \color#000000 32 & \background-color#d6e6f4 \color#000000 24 & \background-color#dceaf6 \color#000000 8 & \background-color#9dcae1 \color#000000 18 & \background-color#f7fbff \color#000000 0 \\
     & UA & \background-color#f7fbff \color#000000 32 & \background-color#eef5fc \color#000000 86 & \background-color#ddeaf7 \color#000000 122 & \background-color#08306b \color#f1f1f1 2174 & \background-color#f7fbff \color#000000 0 & \background-color#c6dbef \color#000000 58 & \background-color#dfebf7 \color#000000 18 & \background-color#99c7e0 \color#000000 23 & \background-color#bfd8ed \color#000000 13 & \background-color#f7fbff \color#000000 0 \\
    \multirow[c]{2}{*}{US} & RU & \background-color#dbe9f6 \color#000000 1976 & \background-color#08306b \color#f1f1f1 1817 & \background-color#08306b \color#f1f1f1 923 & \background-color#f5fafe \color#000000 17 & \background-color#08306b \color#f1f1f1 743 & \background-color#79b5d9 \color#000000 108 & \background-color#105ba4 \color#f1f1f1 122 & \background-color#e7f0fa \color#000000 5 & \background-color#e3eef8 \color#000000 5 & \background-color#f7fbff \color#000000 0 \\
     & UA & \background-color#f7fbff \color#000000 39 & \background-color#d5e5f4 \color#000000 315 & \background-color#deebf7 \color#000000 116 & \background-color#edf4fc \color#000000 112 & \background-color#dfecf7 \color#000000 88 & \background-color#dce9f6 \color#000000 32 & \background-color#b2d2e8 \color#000000 46 & \background-color#f7fbff \color#000000 0 & \background-color#f7fbff \color#000000 0 & \background-color#f7fbff \color#000000 0 \\
    \multirow[c]{2}{*}{DE} & RU & \background-color#f7fbff \color#000000 23 & \background-color#f6faff \color#000000 10 & \background-color#e0ecf8 \color#000000 108 & \background-color#f7fbff \color#000000 0 & \background-color#f7fbff \color#000000 0 & \background-color#f6faff \color#000000 1 & \background-color#f3f8fe \color#000000 3 & \background-color#f1f7fd \color#000000 2 & \background-color#f3f8fe \color#000000 1 & \background-color#f7fbff \color#000000 0 \\
     & UA & \background-color#f7fbff \color#000000 0 & \background-color#f7fbff \color#000000 6 & \background-color#f5f9fe \color#000000 12 & \background-color#f7fbff \color#000000 1 & \background-color#f7fbff \color#000000 0 & \background-color#f7fbff \color#000000 0 & \background-color#f7fbff \color#000000 0 & \background-color#f7fbff \color#000000 0 & \background-color#f7fbff \color#000000 0 & \background-color#f7fbff \color#000000 0 \\
    \multirow[c]{2}{*}{PL} & RU & \background-color#f7fbff \color#000000 2 & \background-color#f7fbff \color#000000 7 & \background-color#9fcae1 \color#000000 345 & \background-color#f7fbff \color#000000 0 & \background-color#f7fbff \color#000000 0 & \background-color#f7fbff \color#000000 0 & \background-color#f6faff \color#000000 1 & \background-color#08306b \color#f1f1f1 59 & \background-color#f7fbff \color#000000 0 & \background-color#f7fbff \color#000000 0 \\
     & UA & \background-color#f7fbff \color#000000 0 & \background-color#f7fbff \color#000000 1 & \background-color#f0f6fd \color#000000 35 & \background-color#f7fbff \color#000000 2 & \background-color#f7fbff \color#000000 0 & \background-color#f7fbff \color#000000 0 & \background-color#f6faff \color#000000 1 & \background-color#d9e7f5 \color#000000 9 & \background-color#f7fbff \color#000000 0 & \background-color#f7fbff \color#000000 0 \\
    \multirow[c]{2}{*}{NL} & RU & \background-color#f7fbff \color#000000 6 & \background-color#f6faff \color#000000 9 & \background-color#eef5fc \color#000000 44 & \background-color#f7fbff \color#000000 3 & \background-color#f7fbff \color#000000 0 & \background-color#bfd8ed \color#000000 63 & \background-color#f3f8fe \color#000000 3 & \background-color#f7fbff \color#000000 0 & \background-color#08306b \color#f1f1f1 48 & \background-color#f7fbff \color#000000 0 \\
     & UA & \background-color#f7fbff \color#000000 0 & \background-color#f7fbff \color#000000 3 & \background-color#f7fbff \color#000000 2 & \background-color#f7fbff \color#000000 3 & \background-color#f7fbff \color#000000 0 & \background-color#f3f8fe \color#000000 5 & \background-color#f7fbff \color#000000 0 & \background-color#f7fbff \color#000000 0 & \background-color#eaf3fb \color#000000 3 & \background-color#f7fbff \color#000000 0 \\
    \multirow[c]{2}{*}{IS} & RU & \background-color#f5fafe \color#000000 152 & \background-color#92c4de \color#000000 733 & \background-color#e1edf8 \color#000000 101 & \background-color#f7fbff \color#000000 5 & \background-color#f7fbff \color#000000 1 & \background-color#cde0f1 \color#000000 49 & \background-color#57a0ce \color#f1f1f1 82 & \background-color#edf4fc \color#000000 3 & \background-color#f3f8fe \color#000000 1 & \background-color#f7fbff \color#000000 0 \\
     & UA & \background-color#f7fbff \color#000000 3 & \background-color#e5eff9 \color#000000 167 & \background-color#f4f9fe \color#000000 15 & \background-color#f2f7fd \color#000000 63 & \background-color#f6faff \color#000000 3 & \background-color#e7f1fa \color#000000 19 & \background-color#e6f0f9 \color#000000 13 & \background-color#f1f7fd \color#000000 2 & \background-color#f7fbff \color#000000 0 & \background-color#d0e1f2 \color#000000 1 \\
    \multirow[c]{2}{*}{JP} & RU & \background-color#f7fbff \color#000000 1 & \background-color#dfecf7 \color#000000 213 & \background-color#2575b7 \color#f1f1f1 675 & \background-color#f7fbff \color#000000 0 & \background-color#f7fbff \color#000000 0 & \background-color#f7fbff \color#000000 0 & \background-color#f2f7fd \color#000000 4 & \background-color#f7fbff \color#000000 0 & \background-color#f7fbff \color#000000 0 & \background-color#f7fbff \color#000000 0 \\
     & UA & \background-color#f7fbff \color#000000 0 & \background-color#f5f9fe \color#000000 26 & \background-color#deebf7 \color#000000 116 & \background-color#f7fbff \color#000000 0 & \background-color#f7fbff \color#000000 0 & \background-color#f7fbff \color#000000 0 & \background-color#f3f8fe \color#000000 3 & \background-color#f7fbff \color#000000 0 & \background-color#f3f8fe \color#000000 1 & \background-color#f7fbff \color#000000 0 \\
    \multirow[c]{2}{*}{SK} & RU & \background-color#f7fbff \color#000000 1 & \background-color#f7fbff \color#000000 0 & \background-color#f7fbff \color#000000 3 & \background-color#f7fbff \color#000000 0 & \background-color#f7fbff \color#000000 0 & \background-color#f7fbff \color#000000 0 & \background-color#f7fbff \color#000000 0 & \background-color#f7fbff \color#000000 0 & \background-color#f7fbff \color#000000 0 & \background-color#08306b \color#f1f1f1 5 \\
     & UA & \background-color#f7fbff \color#000000 0 & \background-color#f7fbff \color#000000 1 & \background-color#f7fbff \color#000000 0 & \background-color#f7fbff \color#000000 0 & \background-color#f7fbff \color#000000 0 & \background-color#f7fbff \color#000000 0 & \background-color#f7fbff \color#000000 0 & \background-color#f7fbff \color#000000 0 & \background-color#f7fbff \color#000000 0 & \background-color#94c4df \color#000000 2 \\
    \end{tabular}
    \caption{Caption}
    \label{tab:my_label}
\end{table}


==> packages.tex <==
\usepackage{float}
\usepackage{booktabs}
\usepackage{multirow}
\usepackage{multicol}
\usepackage{caption}
\usepackage{subfig}
\usepackage[table]{xcolor}

==> sections/conclusion.tex <==
\clearpage
\section{Conclusion}

\RaggedRight \textit{[Yasir]}
\justifying

==> sections/old/introduction.tex <==
\section{Introduction}
\label{sec:introduction}
\hfill \\
\textit{SITUATION}
\\ \\
\textbf{Main idea:} The importance of enterprise cloud services for businesses and organizations
\\ \\
\textbf{Main idea:} Replicated and globally distributed infrastructure of cloud providers increases their resilience (the ability to quickly recover against disruption)
\\ \\
\textbf{Main idea:} On-premise solution requires the user to maintain and minimize disruption to the infra, especially physical disturbance
\break
\\ \\
\textit{COMPLICATION}
\\ \\
\textbf{Main idea:} Despite the advantages, many organizations still hesitate to use cloud due to security, privacy, and governance/policy issue
\\ \\
\textbf{Main idea:} Russian invasion of Ukraine involves attacks on physical infrastructure using missiles and explosives, targeting both residential and governmental area
\\ \\
\textbf{Main idea:} These attacks also threaten IT infra, and might destroy important data and cut critical service when targeting data centers (cite attack on UA server), especially those provided as locally isolated on-premise
\\ \\
\textbf{Main idea:} Organizations relying on IT systems should be concerned about this and react accordingly
\break
\\ \\
\textit{QUESTION}
\\ \\
\textbf{Main idea:} Are organizations aware of this risk and respond to the risk by adopting a more resilient strategy for their IT system? For example, 
\begin{itemize}
    \item by start using cloud services from 3rd party, 
    \item by moving from local to global providers, or 
    \item by start using multiple providers, or
    \item by moving from smaller to bigger cloud providers.
\end{itemize}
% \break
\\ \\
\textit{ANSWER}
\\ \\
\textbf{Main idea:} We want to study how Russian attacks on Ukrainian infrastructure affect cloud consumers in the surrounding area, hence, affect the customer portfolio of the cloud service providers
\\ \\
\textbf{Main idea:} We study this behavior among managed DNS consumers and web hosting consumers
\\ \\
\textbf{Main idea:} We collect historical data of Russian missile/explosive attacks from the newspaper archive
\\ \\
\textbf{Main idea:} We use active DNS measurement data from OpenINTEL to observe the change in the DNS and web hosting practice
\break
\\ \\
\textit{CONTRIBUTIONS}
\\ \\
POINTS OF CONTRIBUTIONS HERE
\\ \\

\subsection{Hypothesis}
\label{sec:hypothesis}

\begin{enumerate}
    \item [H1] Russian attacks on Ukraine increase the number of domain names that start using cloud services from 3$^{rd}$ party providers.
    \item [H2] Russian attacks on Ukraine increase the number of domain names that move from local to international providers.
    \item [H3] Russian attacks on Ukraine increase the number of domain names that move from smaller to bigger service providers.
    \item [H4] Russian attacks on Ukraine increase the number of domain names that start using multiple cloud service providers.
\end{enumerate}
\hfill \\
\textit{SCOPE DEFINITION}
\\ \\
\textbf{Attack}: attacks or attempts launched by Russia targeting physical infrastructure in Ukraine using explosive materials as reported by newspapers from the start of invasion to date.
\\ \\
\textbf{Services}: DNS authoritative service, web hosting service
\\ \\
\textbf{Providers}: top 1k service providers (in the world? in Europe? )
\\ \\
\textbf{Domain names}:
\begin{itemize}
    \item \textbf{ccTLD domains}: domain names under ccTLD of Russia, Ukraine, and surrounding countries (specify! ask Rafaele), OR
    \item \textcolor{red}{\textbf{TBD Hosted or served by local infra}: domain names whose auth NS server or web hosted by infra in Russia, Ukraine, and surrounding countries}
    % \item \textbf{Tenants of the providers}: only domain names that use NS or web servers of the top 1k providers.
\end{itemize}

==> sections/old/methodology.tex <==
\section{Methodology}
\label{sec:methodology}

\subsection{Data Sets}

\subsubsection{Time frame} From February 2022 (start of conflict) to date

\subsubsection{Attack data set} \hfill \\
\textit{Source:} Newspaper articles archived in LexisNexis repository.
\\
\textit{Method:}
\begin{itemize}
    \item Retrieve all newspaper articles containing some keywords (e.g. "ukraine attack") from XXX to XXX
    \item Count the number of articles per day
    \item Peaks indicate actual attacks
    \item Verify with random sampling some articles
\end{itemize}

\subsubsection{Active DNS measurement data set} \hfill \\
\textit{Source:} OpenINTEL
\begin{itemize}
    \item TLDs: 
    \begin{itemize}
        \item Conflicting countries: .ru, .ua (and its cycrillic form)
        \item Surrounding countries (confirm with Raffaele which ccTLDs are now in coverage): .fi (Finland), .sk (Slovakia), .at (Austria), .ee (Estonia), .pl (Poland)
    \end{itemize}
    \item Records:
    \begin{itemize}
        \item NS records: to know the auth NS servers they are using
        \item RTT records: to know if there is a connection problem following the attack (to avoid bias, in case they change providers due to a downtime)
        \item A/AAAA records: to know their web hosting
    \end{itemize}
\end{itemize}
% \break
% \textit{Method:}
% \begin{itemize}
%     \item 
% \end{itemize}

\subsubsection{Metadata}
\begin{itemize}
    \item IP geolocation: to geolocate the auth NS servers and web hosting server
    \item IP-to-ASN-to-Provider: to map auth NS / web servers to the 3rd party provider
    \item Hosting Checker - Find out who is hosting any website
\end{itemize}

\subsubsection{List of service providers} \hfill \\
\textit{Source:}
\begin{itemize}
    \item Managed DNS providers: OpenINTEL NS records, based on total unique domain names served on date, top 1k.
    \item Web hosting providers: (?)
\end{itemize}
% \break
% \textit{Method:}
% \begin{itemize}
%     \item 
% \end{itemize}

\subsubsection{Categorizing domain names} \hfill \\
% Identify which NS is private (on-premise), and which is of 3rd party (outsourced), then label domain names with: 1) All Private, 2) Private and Outsourced, or 3) All Outsourced \hfill \\
\begin{itemize}
    \item Identify if domain names are the tenants of any providers from the list: \textit{1) Customer}, or \textit{2) Non-costumer}.
    \item Identify which domain names use service from single (same SLD for all NS records) or multiple providers (different SLDs) and label whether the domain name use: \textit{1) Single provider}, or \textit{2) Multiple providers}
\end{itemize}

% \subsubsection{Domain names data set}
% All domain names under following ccTLDs (TBC to Rafaele)
% \begin{itemize}
%     \item Conflicting countries: .ru, .ua (and its cycrillic form)
%     \item Surrounding countries: .fi (Finland), .sk (Slovakia), .at (Austria), .ee (Estonia), .pl (Poland)
% \end{itemize}

% \subsubsection{Domain name properties}
% \begin{itemize}
%     \item NS records: to know their auth NS servers they use
%     \item RTT records: to know if there is a connection problem following the attack (might be another trigger of behavior)
%     \item A/AAAA records: to know their web hosting
% \end{itemize}

 

